Continuous Contrastive Learning for Long-Tailed Semi-Supervised Recognition

Long-tailed semi-supervised learning poses a significant challenge in training models with limited labeled data exhibiting a long-tailed label distribution. Current state-of-the-art LTSSL approaches heavily rely on high-quality pseudo-labels for large-scale unlabeled data. However, these methods often neglect the impact of representations learned by the neural network and struggle with real-world unlabeled data, which typically follows a different distribution than labeled data. This paper introduces a novel probabilistic framework that unifies various recent proposals in long-tail learning. Our framework derives the class-balanced contrastive loss through Gaussian kernel density estimation. We introduce a continuous contrastive learning method, CCL, extending our framework to unlabeled data using reliable and smoothed pseudo-labels. By progressively estimating the underlying label distribution and optimizing its alignment with model predictions, we tackle the diverse distribution of unlabeled data in real-world scenarios. Extensive experiments across multiple datasets with varying unlabeled data distributions demonstrate that CCL consistently outperforms prior state-of-the-art methods, achieving over 4% improvement on the ImageNet-127 dataset. Our source code is available at https://github.com/zhouzihao11/CCL

==> Table/cifar100.tex <==
\begin{table*}[t]
\caption{Test accuracy on CIFAR100-LT dataset under $uniform$ and $reversed$ settings. The best results are in \textbf{bold}.}
\label{t4}
\centering
    \begin{tabular}{lcccccccccc}
        \toprule
         & \multicolumn{4}{c}{CIFAR100-LT ($\gamma_l \neq \gamma_u$)} \\
         & \multicolumn{2}{c}{$\gamma_u=1$ (uniform)} & \multicolumn{2}{c}{$\gamma_u=1/10$ (reversed)} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
         \multirow{2}{*}{Algorithm}  & $N_1=50$  & $N_1=150$ & $N_1=50$  & $N_1=150$ \\
        & $M_1=400$ & $M_1=300$ & $M_1=400$ & $M_1=300$ \\
        \cmidrule(r){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} 

        FixMatch~       & \ms{45.5}{0.71}  & \ms{58.1}{0.72} & \ms{44.2}{0.43}  & \ms{57.3}{0.19} \\
        ~~w/ DARP \cite{kim2020distribution}~    & \ms{43.5}{0.95}  & \ms{55.9}{0.32} & \ms{36.9}{0.48}  & \ms{51.8}{0.92}\\
        ~~w/ CReST \cite{wei2021crest}~   & \ms{43.5}{0.30}  & \ms{59.2}{0.25} & \ms{39.0}{1.11} & \ms{56.4}{0.62} \\
        ~~w/ CReST+ \cite{wei2021crest}~  & \ms{43.6}{1.60}  & \ms{58.7}{0.16} & \ms{39.1}{0.77} & \ms{56.4}{0.78} \\
        ~~w/ DASO \cite{oh2022daso}     & \ms{53.9}{0.66} & \ms{61.8}{0.98} & \ms{51.0}{0.19} & \ms{60.0}{0.31}  \\
        ~~w/ ACR \cite{wei2023towards}      & \ms{57.9}{0.78} & \ms{65.8}{0.99} & \ms{51.7}{0.11} & \ms{63.0}{0.17} \\
        ~~w/ CPE \cite{ma2024three}      & \ms{-}{-} & \ms{-}{-} & \ms{-}{-} & \ms{-}{-} \\
        \rowcolor{gray!20}
        ~~w/ \textbf{Ours}                       &
        \msb{59.8}{0.28} &
        \msb{67.9}{0.70} &
        \msb{54.1}{0.14} &
        \msb{64.7}{0.22} \\    
        \bottomrule
    \end{tabular}%
% \vspace{-2mm}
\end{table*}

==> Table/imgnet.tex <==
% \begin{table}[ht]\
% \caption{Test accuracy on ImageNet-127 dataset. The best results are in \textbf{bold}.}
% \label{t5}
% \centering
% \footnotesize
% \begin{tabular}{llccl}
% \toprule
% % &&Small-ImageNet
% \multicolumn{5}{c}{Small-ImageNet}
% \\\cmidrule(r){1-4}
% Algorithm   &  & $32 \times 32$    & $64 \times 64$    &                      \\ \cmidrule(r){1-1} \cmidrule(lr){3-4}
% \begin{tabular}[c]{l}FixMatch\\ 
% \quad w/ DARP \cite{kim2020distribution}\\ \quad w/ DARP+cRT\\ 
% \quad w/ CReST+\\ \quad w/ CReST++LA\\ 
% \quad w/ CoSSL\\ \quad w/ TRAS\\ 
% \quad w/ ACR\\
% \quad w/ CPE\\
% \rowcolor{gray!20}
% \quad w/ \textbf{Ours}
% \end{tabular} &  & \begin{tabular}[c]{c}29.7\\ 30.5\\ 39.7\\ 32.5\\ 40.9\\ 43.7\\ 46.2\\ 57.2 \\ - \\ \textbf{61.5}\end{tabular} & \begin{tabular}[c]{c}42.3\\ 42.5\\ 51.0\\ 44.7\\ 55.9\\ 53.9\\ 54.1\\ 63.6  \\ -\\ \textbf{--(\textcolor{red}{+--})}\end{tabular} & \multicolumn{1}{c}{} \\ 
% \bottomrule
% \end{tabular}%
% \end{table}
\begin{table}[ht]
\caption{Test accuracy on ImageNet-127 dataset. The best results are in \textbf{bold}.}
\label{t5}
\centering
\footnotesize
\begin{tabular}{llccl}
\toprule
\multicolumn{5}{c}{Small-ImageNet} \\
\cmidrule(r){1-4}
Algorithm & & $32 \times 32$ & $64 \times 64$ & \\
\cmidrule(r){1-1} \cmidrule(lr){3-4}
FixMatch & & 29.7 & 42.3 & \\
\quad w/ DARP \cite{kim2020distribution} & & 30.5 & 42.5 & \\
\quad w/ DARP+cRT \cite{kim2020distribution}& & 39.7 & 51.0 & \\
\quad w/ CReST+ \cite{wei2021crest}& & 32.5 & 44.7 & \\
\quad w/ CReST++LA \cite{wei2021crest}& & 40.9 & 55.9 & \\
\quad w/ CoSSL \cite{fan2022cossl}& & 43.7 & 53.9 & \\
\quad w/ TRAS \cite{wei2022transfer}& & 46.2 & 54.1 & \\
\quad w/ ACR \cite{wei2023towards}& & 57.2 & 63.6 & \\
\quad w/ CPE \cite{ma2024three}& & - & - & \\
\rowcolor{gray!20}
\quad  w/ \textbf{CCL} & & \textbf{61.5} & \textbf{--} & \\
\bottomrule
\end{tabular}
\end{table}

